GPU Load Balancing

Fine-grained workload and resource balancing is the key to high performance for regular and irregular computations on the GPUs. In this dissertation, we conduct an extensive survey of existing load-balancing techniques to build an abstraction that addresses the difficulty of scheduling computations on the GPU. We propose a GPU fine-grained load-balancing abstraction that decouples load balancing from work processing and aims to support both static and dynamic schedules with a programmable interface to implement new load-balancing schedules. Prior to our work, the only way to unleash the GPU's potential on irregular problems has been to workload-balance through application-specific, tightly coupled load-balancing techniques. With our open-source framework for load-balancing, we hope to improve programmers' productivity when developing irregular-parallel algorithms on the GPU, and also improve the overall performance characteristics for such applications by allowing a quick path to experimentation with a variety of existing load-balancing techniques. Using our insights from load-balancing irregular workloads, we build Stream-K, a work-centric parallelization of matrix multiplication (GEMM) and related computations in dense linear algebra. Whereas contemporary decompositions are primarily tile-based, our method operates by partitioning an even share of the aggregate inner loop iterations among physical processing elements. This provides a near-perfect utilization of computing resources, regardless of how efficiently the output tiling for any given problem quantizes across the underlying processing elements. On GPU processors, our Stream-K parallelization of GEMM produces a peak speedup of up to 14x and 6.7x, and an average performance response that is both higher and more consistent across 32K GEMM problem geometries than state-of-the-art math libraries such as CUTLASS and cuBLAS.

==> ch_loadbalance/chapters/abstract.tex <==
%% Abstract
%% Note: \begin{abstract}...\end{abstract} environment must come
%% before \maketitle command
\begin{abstract}
    % We propose to build an open-source GPU load-balancing framework for applications that exhibit irregular parallelism. The set of applications and algorithms we consider are fundamental to computing tasks ranging from sparse machine learning, large numerical simulations, and on through to graph analytics. The underlying data and data structures that drive these applications exhibit access patterns that naturally don't map well to the GPU's architecture that is designed with dense and regular access patterns in mind. Prior to the work we present and propose here, the only way to unleash the GPU's full power on these problems has been to workload balance through tightly coupled load-balancing techniques.

    We propose a GPU fine-grained load-balancing abstraction that decouples load balancing from work processing and aims to support both static and dynamic schedules with a programmable interface to implement new load-balancing schedules. Prior to our work, the only way to unleash the GPU's potential on irregular problems has been to workload-balance through application-specific, tightly coupled load-balancing techniques.

    With our open-source framework for load-balancing, we hope to improve programmers' productivity when developing irregular-parallel algorithms on the GPU, and also improve the overall performance characteristics for such applications by allowing a quick path to experimentation with a variety of existing load-balancing techniques. Consequently, we also hope that by separating the concerns of load-balancing from work processing within our abstraction, managing and extending existing code to future architectures becomes easier.
\end{abstract}


==> ch_loadbalance/chapters/acknowledgements.tex <==
%% Acknowledgments
\begin{acks}                            %% acks environment is optional
    %% contents suppressed with 'anonymous'
%% Commands \grantsponsor{<sponsorID>}{<name>}{<url>} and
%% \grantnum[<url>]{<sponsorID>}{<number>} should be used to
%% acknowledge financial support and will be used by metadata
%% extraction tools.
This material is based upon work supported by the
\grantsponsor{GS100000001}{National Science
Foundation}{http://dx.doi.org/10.13039/100000001} under Grant
No.~\grantnum{GS100000001}{nnnnnnn} and Grant
No.~\grantnum{GS100000001}{mmmmmmm}.  Any opinions, findings, and
conclusions or recommendations expressed in this material are those
of the author and do not necessarily reflect the views of the
National Science Foundation.
\end{acks}

==> ch_streamk_v2/chapters/abstract.tex <==
\begin{abstract}
  We introduce \emph{Stream-K}, a work-centric parallelization of matrix
  multiplication (GEMM) and related computations in dense linear algebra.
  Whereas contemporary decompositions are primarily tile-based, our method
  operates by partitioning an even share of the aggregate inner loop
  iterations among physical processing elements. This provides a
  near-perfect utilization of computing resources, regardless of how
  efficiently the output tiling for any given problem quantizes across the
  underlying processing elements.

  On GPU processors, our \emph{Stream-K} parallelization of GEMM produces
  a peak speedup of up to 14$\times$ and 6.7$\times$, and an average performance response that is both higher and more consistent
  across 32,824 GEMM problem geometries than state-of-the-art
  math libraries such as CUTLASS and cuBLAS\@. Furthermore, we achieve this performance
  from a \emph{single} tile size configuration per floating-point precision, whereas today's math libraries
  employ complex kernel-selection heuristics to select from a large
  ensemble of kernel variants.
\end{abstract}

==> ch_survey/chapters/abstract.tex <==
\begin{abstract}
    A clear and well-documented \LaTeX\ document is presented as an
    article formatted for publication by ACM in a conference proceedings
    or journal publication. Based on the ``acmart'' document class, this
    article presents and explains many of the common variations, as well
    as many of the formatting elements an author may use in the
    preparation of the documentation of their work.
\end{abstract}


==> ch_survey/chapters/acknowledgement.tex <==
\begin{acks}
    Identification of funding sources and other support, and thanks to
    individuals and groups that assisted in the research and the
    preparation of the work should be included in an acknowledgment
   chapter, which is placed just before the reference chapter in your
    document. \mosama{@jowens chapter.}\\ 
Matt Drescher---comments\\
Julian Shun---comments\\
Serban D. Porumbescu---guidance
\end{acks}


==> ch_survey/chapters/appendices.tex <==
\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
\begin{verbatim}
  \appendix
\end{verbatim}
and note that in the appendix, chapter are lettered, not
numbered. This document has two appendices, demonstrating the chapter
and subsection identification method.

==> ch_survey/chapters/extended_abstract.tex <==
\section{SIGCHI Extended Abstracts}

The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
not in Word) produces a landscape-orientation formatted article, with
a wide left margin. Three environments are available for use with the
``\verb|sigchi-a|'' template style, and produce formatted output in
the margin:
\begin{itemize}
    \item {\verb|sidebar|}:  Place formatted text in the margin.
    \item {\verb|marginfigure|}: Place a figure in the margin.
    \item {\verb|margintable|}: Place a table in the margin.
\end{itemize}

==> ch_survey/chapters/irregular.tex <==
\section{Irregular Problem Space}
\label{sec:irregular-problem-space}

Using the characterization described in Chapter~\ref{sec:load-balancing-taxonomy} and~\ref{sec:deeper-dive}, we can make recommendations of workload balancing techniques for a given irregular problem. We describe this irregular-parallel problem space approximately as a tree and tree traversal problem. \jowens{How you are organizing this as a tree is totally not clear from the preceding sentence. This needs a lot more explanation.} Our assumption is that any level of the tree, each element can be traversed in parallel. This is not always true, but it is true in the problems we think about. \jowens{``We think about''? Can you distinguish what kind of problems have this property and which don't?} For instance, vertices in a Breadth-First Search (BFS) algorithm or rows in a sparse-matrix multiplication. With each property of the tree structure of the traversal described below, we recommend either types of techniques (described in the taxonomy in Chapter~\ref{sec:load-balancing-taxonomy}), or a specific implementation of the technique (described in Chapter~\ref{sec:deeper-dive}) best suited for the problem based on previous publications. For cases where there is no previous publication discussing the tradeoff of a technique for a given problem, we recommend a path to discovering a suitable solution.

\jowens{Try to eliminate each use of the word ``you'' in the below text.}

\subsection{Tree Structure}
\label{sec:tree-structure}
Similar to Chapter~\ref{sec:static-dynamic}, we determine for a irregular problem described as a tree: Is the tree structure determined before any traversal starts, or is it discovered/generated along the way? An example of a static tree structure is a sparse matrix, where one can look at the sparse matrix and know exactly what the traversal will be, and CSR is designed to make that staticness \jowens{instead of ``staticness'', ``traversal structure''?} explicit. Dynamic tree structures, however, have two different modes:
\begin{enumerate}
  \item Dynamic where the data structure does not explicitly show the entire structure but the traversal is still determined at ``compile'' time. A push-based BFS where the traversal goes from source to neighboring vertices would be an example of this type of dynamic structure. The tree traversal is completely determined at compile time, but that's not evident in the data structure at all (e.g., you cannot look at the data structure and tell how deep the tree is, i.e., the diameter of the graph).
  \item Dynamic where the traversal order is not available at compile time at all, where the traversal is completely dynamically generated (and possibly new nodes are created during the traversal). Recursive surface subdivision (e.g., Catmull-Clark subdivision) would be in this category. This type of dynamic is equivalent to ``creating work during traversal'', in contrast to the previous bullet, which does not create new work to do (e.g., in push BFS, the upper bound of the amount of work is approximately capped at compile time and modulo redundant node visits, you visit every vertex only once).
\end{enumerate}

\jowens{I think I'd try to name and divide the above subsection as three separate things rather than one static and a subclass of two dynamics. Static/obvious; dynamic/discovered; dynamic/generated?}

The advantage of static is that you can possibly do compile-time optimizations and/or pick an appropriate load-balance strategy at compile time instead of figuring it out only after the traversal begins. All load-balancing techniques characterized as ``Static'' in Tables~\ref{tab:annotated-bib}--\ref{tab:annotated-bib_2} are viable approaches for solving load-imbalance issues for problems that have a static tree structure, or a dynamic tree structure that does not involve work generation. However, applying static load-balancing schedules to a dynamic tree structure where work is being created during the traversal is a more complicated challenge. One approach is to generate work until a fixed amount of work threshold is reached (effectively turning a dynamic tree structure to a static tree structure), and then apply a static load-balancing strategy to this window of work. Another approach for load balancing dynamic tree structure problems are techniques characterized as ``Dynamic'' in Tables~\ref{tab:annotated-bib}--\ref{tab:annotated-bib_2}. \jowens{Maybe have a sentence on how these techniques, collectively, address the problem.} Task-oriented schedules described in Chapter~\ref{sec:task-oriented-scheduling} are a suitable candidate for tree traversals where work is generated dynamically, as the new work can be queued up and executed as the traversal continues.

\begin{figure}
  \centering
  \includegraphics[page=1,width=\columnwidth]{figs/irregular_problem_space.pdf}
  \caption{Describes which characterization of load-balancing techniques is well-suited for a given irregular problem space as a tree structure/traversal.} \label{fig:tree-structure}
\end{figure}

\subsection{Depth}
How many levels of traversal are there? Matrices for example are 2, tensors can be larger than 2.
Interesting question: are all leaves at the maximum depth?
Your categorization of ``fixed depth'', for me, is ``if I write code to traverse this tree, can I assume the depth is constant for any input''. Sparse matrix, yes. Bipartite graph, yes. BFS, no.

\subsection{Branching Factor}
\label{sec:branching-factor}
The branching factor of the tree is the distribution of the number of children per node, across all nodes. For GPUs, the branching factor of an irregular problem space is the primary factor for deciding which load-balancing algorithm is most appropriate---different degree distributions motivate different load-balancing algorithms~\cite{Yang:2018:DPF,Gale:2020:SGK}. The important questions to ask for a given irregular problem are:
\begin{itemize}
  \item Is the branching factor constant (per-level, at all levels)? For example, a B-tree would have approximately a constant branching factor at all levels (or at least bounded). A non-square matrix would be constant per level but not across levels. Most graphs would not be constant at all.
  \item What is the distribution of branching factors?
  \begin{itemize}
    \item What is the mean branching factor? (Road-like networks $<$ scale-free graphs.) \todo{cite}
    \item What is the standard deviation? (Scale-free graphs would have a large standard deviation, for instance. \todo{indeed, it can be infinite, cite Newman})
    % \item Can we bound it (max/min)? In a well-formed mesh, for instance, the number of neighbors (branching factor) should be no more than six.
  \end{itemize}
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[page=2,width=\columnwidth]{figs/irregular_problem_space.pdf}
  \caption{Describes which load-balancing algorithm to choose for a given distribution of the branching factor. \jowens{For this figure (possibly the other one, but definitely this one), might it be useful to extend it to a full page width and for each arrow, label (briefly) why that decision was made? Might be easier to make the flowchart flow from top to bottom rather than left to right if you do that.}} \label{fig:branching-factor}
\end{figure}

\mosama{@jowens please see if the general idea above makes sense, if not, an easier way to structure this is using the ``Evaluation'' box per schedule in the previous chapter and then just using simple flow-charts to summarize the landscape (like in Figure~\ref{fig:branching-factor} and~\ref{fig:tree-structure}).}

\jowens{I think you're doing this right. Start with the figures and if you have one (two) that makes sense, which you do, structure the narrative around that.}

\subsection{Task-centric Systems}
\jowens{It's interesting to think about how the above points differ when considering a task-centric system rather than a data-parallel (data-centric) one. For instance, data-centric systems generally are going to be level-synchronous (an inherent barrier between each different depth), whereas a task-centric system potentially can have more flexible ordering so long as dependencies are met. (For instance, a task-centric system can do a DFS [perhaps multiple DFSes in parallel], whereas that seems a lot harder with a data-centric system.)} \mosama{I don't currently have a good way to fit this within the current draft of this chapter. I think it is partially addressed when we talk about the tree structure and how dynamic tree structure where work is generated is well suited for task-oriented scheduling.} \jowens{I think I'd like to suggest making this its own chapter. You can explicitly leave questions from this chapter unanswered (dynamic work generation) and then use a new chapter on task-centric systems and load balancing to answer them. I think it's fair to say that you're not going to completely cover the entire topic of task-centered systems in this paper/section, but at least you can focus on the load-balancing aspect. In particular, contrasting task-centric vs. data-centric load balancing is a must (pros/cons). Then the task-centric chapter can stand alone. I would introduce it as ``here's a problem or a couple of problems where data-centric seems like a poor fit, so let's take a step back and think about a different programming model that might be a better fit for these problems''.}


==> ch_survey/chapters/performance.tex <==
\section{Performance Characterization (maybe)}
